On multi-robot search for a stationary object

Two variants of multi-robot search for a stationary object in a priori known environment represented by a graph are studied in the paper. The first one is a generalization of the Traveling Deliveryman Problem where more than one deliveryman is allowed to be used in a solution. Similarly, the second variant is a generalization of the Graph Search Problem. A novel heuristics suitable for both problems is proposed which is furthermore integrated into a cluster-first route second approach. A set of computational experiments was conducted over the benchmark instances derived from the TSPLIB library. The results obtained show that even a standalone heuristics significantly outperforms the standard solution based on k- means clustering in quality of results as well as computational time. The integrated approach furthermore improves solutions found by a standalone heuristics by up to 15% at the expense of higher computational complexity.

==> table-gsp.tex <==
\begin{table*}
\label{tbl:comparison}
\begin{center}
\footnotesize
\begin{tabular}{crrp{0.01em}rrp{0.01em}rrrrp{0.01em}rrrr}
\toprule
Problem & R & BKS & & \multicolumn{2}{c}{Greedy} & & \multicolumn{4}{c}{GrWDMP} & & \multicolumn{4}{c}{kmeans}  \\
&~~ & & & PDB \hfil\hfil &  T\hfil\hfil & & PDB & PDM & SD\hfil\hfil &  T\hfil\hfil &  & PDB & PDM & SD\hfil\hfil &  T\hfil\hfil\\
\midrule
\multirow{5}*{berlin52}
 & 2 & 1289.3665 
 & & 15.49 & 0.29
 & & 2.55 & 2.55  & 0.06 & 55.73
 & & \textbf{0.00} & 7.67  & 101.55 & 65.39
\\
 & 4 & 711.9565 
 & & 8.92 & 0.32
 & & \textbf{0.00} & 0.00  & 0.00 & 24.22
 & & 5.10 & 9.70  & 23.96 & 40.98
\\
 & 6 & 569.3354 
 & & 1.28 & 0.33
 & & \textbf{0.00} & 0.00  & 0.00 & 11.74
 & & 8.06 & 11.66  & 12.52 & 21.95
\\
 & 8 & 510.9161 
 & & 2.82 & 0.36
 & & \textbf{0.00} & 0.00  & 0.00 & 8.35
 & & 4.91 & 9.25  & 14.94 & 14.45
\\
 & 10 & 462.7143 
 & & 0.00 & 0.38
 & & \textbf{0.00} & 0.00  & 0.00 & 4.53
 & & 9.43 & 13.30  & 16.38 & 10.43
\\
\midrule
\multirow{5}*{bier127}
 & 2 & 16938.3426 
 & & 16.94 & 0.92
 & & \textbf{0.00} & 0.58  & 59.14 & 465.85
 & & 1.19 & 9.68  & 1212.99 & 613.18
\\
 & 4 & 9015.8078 
 & & 10.15 & 0.78
 & & \textbf{0.00} & 0.11  & 7.17 & 179.04
 & & 6.09 & 21.01  & 774.75 & 301.05
\\
 & 6 & 6439.1727 
 & & 5.06 & 0.81
 & & \textbf{0.00} & 0.00  & 0.25 & 112.68
 & & 14.08 & 23.26  & 368.25 & 221.56
\\
 & 8 & 5297.5682 
 & & 2.33 & 0.86
 & & \textbf{0.00} & 0.00  & 0.00 & 63.20
 & & 10.91 & 22.10  & 280.29 & 153.78
\\
 & 10 & 4517.5042 
 & & 1.83 & 0.94
 & & \textbf{0.00} & 0.00  & 0.00 & 42.99
 & & 15.53 & 24.25  & 161.22 & 120.06
\\
\midrule
\multirow{5}*{gil262}
 & 2 & 557.1953 
 & & 12.84 & 3.46
 & & \textbf{0.00} & 1.03  & 2.38 & 3465.02
 & & 0.39 & 3.18  & 11.40 & 4415.25
\\
 & 4 & 324.9695 
 & & 8.78 & 2.51
 & & \textbf{0.00} & 0.30  & 0.49 & 1028.91
 & & 9.60 & 10.06  & 1.77 & 2628.16
\\
 & 6 & 241.1403 
 & & 5.21 & 2.49
 & & \textbf{0.00} & 0.12  & 0.16 & 604.07
 & & 13.62 & 17.69  & 6.33 & 1410.60
\\
 & 8 & 208.0251 
 & & 4.62 & 2.57
 & & \textbf{0.00} & 0.03  & 0.06 & 378.99
 & & 15.12 & 20.39  & 6.27 & 1009.05
\\
 & 10 & 195.8603 
 & & 1.75 & 2.89
 & & \textbf{0.00} & 0.00  & 0.00 & 315.60
 & & 13.94 & 18.16  & 4.62 & 788.35
\\
\midrule
\multirow{5}*{lin318}
 & 2 & 9729.8214 
 & & 17.30 & 4.85
 & & 5.48 & 6.23  & 40.37 & 6412.44
 & & \textbf{0.00} & 1.41  & 46.65 & 6757.29
\\
 & 4 & 5614.8969 
 & & 9.26 & 3.67
 & & \textbf{0.00} & 0.40  & 8.24 & 1769.25
 & & 1.00 & 5.74  & 112.89 & 2510.83
\\
 & 6 & 4390.3071 
 & & 4.68 & 3.52
 & & \textbf{0.00} & 0.16  & 3.95 & 878.58
 & & 2.62 & 7.51  & 118.88 & 1773.18
\\
 & 8 & 3728.5347 
 & & 4.50 & 3.77
 & & \textbf{0.00} & 0.02  & 0.75 & 606.11
 & & 5.42 & 9.02  & 135.38 & 1315.97
\\
 & 10 & 3504.8153 
 & & 4.69 & 4.13
 & & \textbf{0.00} & 0.01  & 0.43 & 547.21
 & & 2.99 & 5.94  & 96.50 & 1001.21
\\
\midrule
\multirow{5}*{pcb442}
 & 2 & 11670.8481 
 & & 11.20 & 10.06
 & & 3.23 & 4.25  & 45.68 & 13903.57
 & & \textbf{0.00} & 3.06  & 155.85 & 19525.87
\\
 & 4 & 6076.4795 
 & & 5.80 & 7.07
 & & \textbf{0.00} & 0.39  & 10.10 & 3348.96
 & & 14.86 & 15.81  & 22.50 & 8445.16
\\
 & 6 & 4438.6460 
 & & 4.89 & 6.70
 & & \textbf{0.00} & 0.19  & 3.57 & 1725.01
 & & 17.89 & 21.13  & 70.81 & 5055.13
\\
 & 8 & 3634.2044 
 & & 3.33 & 7.01
 & & \textbf{0.00} & 0.05  & 1.21 & 1113.55
 & & 22.60 & 24.91  & 61.11 & 3643.70
\\
 & 10 & 3197.8358 
 & & 3.34 & 7.64
 & & \textbf{0.00} & 0.01  & 0.39 & 733.25
 & & 24.93 & 28.05  & 47.30 & 2869.68
\\
\midrule
\multirow{5}*{pr1002}
 & 2 & 60325.4178 
 & & 17.21 & 54.04
 & & \textbf{0.00} & 1.22  & 266.22 & 242200.87
 & & 1.78 & 3.06  & 289.47 & 271763.71
\\
 & 4 & 34423.7763 
 & & 20.83 & 36.08
 & & 5.10 & 5.62  & 98.06 & 52536.92
 & & \textbf{0.00} & 0.99  & 137.73 & 77147.53
\\
 & 6 & 25056.6643 
 & & 12.34 & 34.25
 & & \textbf{0.00} & 0.32  & 39.35 & 33415.13
 & & 3.26 & 4.06  & 236.43 & 49881.61
\\
 & 8 & 20813.4050 
 & & 9.51 & 34.61
 & & \textbf{0.00} & 0.24  & 23.37 & 19364.56
 & & 4.46 & 6.70  & 456.05 & 35652.01
\\
 & 10 & 17750.8518 
 & & 9.21 & 38.10
 & & \textbf{0.00} & 0.20  & 15.70 & 11952.95
 & & 5.79 & 8.58  & 491.02 & 25752.29
\\
\midrule
\multirow{5}*{rat575}
 & 2 & 1624.6539 
 & & 12.92 & 17.25
 & & \textbf{0.00} & 1.14  & 8.45 & 29891.17
 & & 0.50 & 1.17  & 5.19 & 50161.28
\\
 & 4 & 885.9464 
 & & 12.11 & 11.67
 & & \textbf{0.00} & 0.46  & 2.41 & 8358.31
 & & 4.77 & 8.81  & 20.46 & 20297.80
\\
 & 6 & 647.9221 
 & & 5.97 & 11.25
 & & \textbf{0.00} & 0.33  & 1.11 & 4596.77
 & & 5.93 & 8.06  & 14.37 & 11989.79
\\
 & 8 & 527.9039 
 & & 5.70 & 11.55
 & & \textbf{0.00} & 0.14  & 0.32 & 2678.61
 & & 9.93 & 11.43  & 7.55 & 8496.11
\\
 & 10 & 444.0691 
 & & 3.56 & 12.76
 & & \textbf{0.00} & 0.10  & 0.21 & 1842.64
 & & 15.72 & 19.20  & 7.37 & 6800.49
\\
\midrule
\multirow{5}*{u724}
 & 2 & 10053.0689 
 & & 20.39 & 27.42
 & & 1.63 & 3.08  & 47.51 & 64240.43
 & & \textbf{0.00} & 0.85  & 31.56 & 87189.09
\\
 & 4 & 5492.4174 
 & & 12.34 & 18.58
 & & \textbf{0.00} & 0.52  & 14.49 & 16706.83
 & & 2.46 & 5.66  & 95.87 & 31098.84
\\
 & 6 & 3967.1502 
 & & 9.06 & 17.38
 & & \textbf{0.00} & 0.35  & 4.86 & 10488.02
 & & 7.99 & 9.06  & 39.43 & 18807.40
\\
 & 8 & 3377.1366 
 & & 6.68 & 18.08
 & & \textbf{0.00} & 0.14  & 2.61 & 6682.94
 & & 8.28 & 9.73  & 24.42 & 13853.41
\\
 & 10 & 2805.0308 
 & & 4.43 & 20.14
 & & \textbf{0.00} & 0.10  & 1.27 & 4474.89
 & & 16.32 & 17.96  & 30.07 & 10550.73
\\
\midrule
\end{tabular}
\end{center}
\caption{Comparison of the greedy approach and the proposed algorithm.}
\end{table*}


==> table-tdp.tex <==
\begin{table*}

\begin{center}
\footnotesize
\begin{tabular}{crr|p{0.01em}rr|p{0.01em}rrrr|p{0.01em}rrrr}
\toprule
Problem & R & BKS & & \multicolumn{2}{c}{clustering} & & \multicolumn{4}{c}{proposed} & & \multicolumn{4}{c}{k-means}  \\
&~~ & & & PDB \hfil\hfil &  T\hfil\hfil & & PDB & PDM & SD\hfil\hfil &  T\hfil\hfil &  & PDB & PDM & SD\hfil\hfil &  T\hfil\hfil\\
\midrule
\multirow{5}*{berlin52}
 & 2 & 70235 
 & & 3.98 & 0.24
 & & \textbf{0.00} & 0.00  & 0.79 & 42.67
 & & 6.82 & 15.76  & 6070.62 & 64.03
\\
 & 4 & 39746 
 & & 0.78 & 0.25
 & & \textbf{0.00} & 0.00  & 0.00 & 19.68
 & & 8.84 & 12.77  & 1052.73 & 31.31
\\
 & 6 & 30563 
 & & 0.03 & 0.27
 & & \textbf{0.00} & 0.00  & 0.00 & 8.75
 & & 14.24 & 18.07  & 824.95 & 17.48
\\
 & 8 & 25470 
 & & 1.34 & 0.30
 & & \textbf{0.00} & 0.00  & 0.00 & 6.61
 & & 13.53 & 21.11  & 1137.95 & 12.69
\\
 & 10 & 23919 
 & & 1.01 & 0.35
 & & \textbf{0.00} & 0.00  & 0.00 & 5.14
 & & 14.83 & 19.05  & 742.42 & 8.96
\\
\midrule
\multirow{5}*{bier127}
 & 2 & 2354332 
 & & 10.03 & 0.78
 & & 1.59 & 2.74  & 8388.61 & 396.88
 & & \textbf{0.00} & 7.66  & 142517.02 & 540.77
\\
 & 4 & 1228367 
 & & 13.10 & 0.64
 & & 5.84 & 5.84  & 0.00 & 116.97
 & & \textbf{0.00} & 16.83  & 80731.98 & 251.61
\\
 & 6 & 879448 
 & & 4.95 & 0.65
 & & \textbf{0.00} & 0.00  & 0.00 & 82.52
 & & 17.52 & 24.22  & 47044.46 & 183.57
\\
 & 8 & 713125 
 & & 0.97 & 0.66
 & & \textbf{0.00} & 0.00  & 0.00 & 52.17
 & & 14.96 & 23.25  & 27229.50 & 122.54
\\
 & 10 & 612336 
 & & 0.35 & 0.73
 & & \textbf{0.00} & 0.00  & 0.00 & 38.65
 & & 19.48 & 26.01  & 18738.51 & 99.08
\\
\midrule
\multirow{5}*{gil262}
 & 2 & 153716 
 & & 8.66 & 3.23
 & & \textbf{0.00} & 0.98  & 601.31 & 3055.23
 & & 0.06 & 4.32  & 3130.36 & 4342.95
\\
 & 4 & 87114 
 & & 6.96 & 2.16
 & & \textbf{0.00} & 0.21  & 81.67 & 1019.36
 & & 12.65 & 13.30  & 209.34 & 2187.43
\\
 & 6 & 65428 
 & & 3.10 & 2.07
 & & \textbf{0.00} & 0.04  & 22.76 & 599.17
 & & 13.56 & 18.98  & 2124.00 & 1168.37
\\
 & 8 & 55306 
 & & 1.90 & 2.10
 & & \textbf{0.00} & 0.01  & 8.14 & 447.16
 & & 16.25 & 21.84  & 1566.33 & 776.67
\\
 & 10 & 50292 
 & & 0.75 & 2.18
 & & \textbf{0.00} & 0.00  & 2.63 & 329.39
 & & 19.43 & 23.64  & 1417.02 & 617.23
\\
\midrule
\multirow{5}*{lin318}
 & 2 & 3140312 
 & & 15.07 & 4.29
 & & 4.55 & 5.75  & 15004.90 & 5855.93
 & & \textbf{0.00} & 2.92  & 32535.88 & 5931.95
\\
 & 4 & 1811206 
 & & 6.46 & 2.92
 & & \textbf{0.00} & 0.24  & 2817.56 & 1644.35
 & & 1.80 & 7.44  & 36532.68 & 2239.29
\\
 & 6 & 1431946 
 & & 4.18 & 2.86
 & & \textbf{0.00} & 0.08  & 1004.02 & 940.59
 & & 2.35 & 5.92  & 31411.96 & 1371.37
\\
 & 8 & 1214427 
 & & 3.24 & 2.85
 & & \textbf{0.00} & 0.03  & 292.51 & 563.80
 & & 4.56 & 8.13  & 44304.42 & 976.14
\\
 & 10 & 1129348 
 & & 3.93 & 3.03
 & & \textbf{0.00} & 0.01  & 256.28 & 565.05
 & & 3.55 & 6.49  & 27180.85 & 760.35
\\
\midrule
\multirow{5}*{pcb442}
 & 2 & 5292831 
 & & 5.07 & 9.13
 & & \textbf{0.00} & 0.56  & 17515.61 & 14006.46
 & & 5.56 & 6.46  & 26968.07 & 24343.18
\\
 & 4 & 2849704 
 & & 4.96 & 6.08
 & & \textbf{0.00} & 0.44  & 7294.97 & 3758.14
 & & 14.27 & 14.61  & 6929.25 & 8974.81
\\
 & 6 & 2055340 
 & & 2.07 & 5.75
 & & \textbf{0.00} & 0.14  & 2272.75 & 1641.71
 & & 17.98 & 21.26  & 33959.70 & 4861.82
\\
 & 8 & 1607307 
 & & 1.65 & 5.73
 & & \textbf{0.00} & 0.11  & 1234.00 & 1251.63
 & & 26.51 & 30.42  & 30783.56 & 3115.88
\\
 & 10 & 1402893 
 & & 2.74 & 5.84
 & & \textbf{0.00} & 0.05  & 898.36 & 988.54
 & & 29.37 & 33.29  & 24376.01 & 2261.04
\\
\midrule
\multirow{5}*{rat575}
 & 2 & 994166 
 & & 7.01 & 16.96
 & & \textbf{0.00} & 0.96  & 3631.90 & 37961.41
 & & 2.20 & 3.10  & 3053.47 & 66531.58
\\
 & 4 & 524957 
 & & 6.65 & 10.47
 & & \textbf{0.00} & 0.50  & 1110.60 & 9644.29
 & & 9.78 & 13.40  & 12210.99 & 23472.77
\\
 & 6 & 375842 
 & & 6.60 & 10.20
 & & \textbf{0.00} & 0.22  & 375.69 & 4100.55
 & & 11.89 & 13.89  & 8107.88 & 11401.33
\\
 & 8 & 303082 
 & & 3.46 & 10.10
 & & \textbf{0.00} & 0.06  & 137.15 & 2312.13
 & & 15.63 & 17.79  & 5449.48 & 7426.09
\\
 & 10 & 260937 
 & & 1.37 & 10.47
 & & \textbf{0.00} & 0.05  & 101.79 & 1406.92
 & & 18.82 & 22.19  & 4480.78 & 5577.58
\\
\midrule
\multirow{5}*{u724}
 & 2 & 7479059 
 & & 8.28 & 26.90
 & & \textbf{0.00} & 1.31  & 39681.60 & 57579.28
 & & 2.86 & 3.47  & 24549.00 & 79037.02
\\
 & 4 & 3904506 
 & & 7.77 & 17.47
 & & \textbf{0.00} & 0.52  & 8792.00 & 16542.24
 & & 9.23 & 12.04  & 59939.66 & 26556.46
\\
 & 6 & 2926359 
 & & 5.31 & 16.85
 & & \textbf{0.00} & 0.38  & 4477.46 & 8135.85
 & & 10.39 & 11.53  & 22159.80 & 15149.82
\\
 & 8 & 2427262 
 & & 4.49 & 17.03
 & & \textbf{0.00} & 0.11  & 1496.06 & 6363.60
 & & 11.95 & 13.89  & 28998.38 & 10828.30
\\
 & 10 & 2111492 
 & & 2.46 & 17.42
 & & \textbf{0.00} & 0.12  & 1014.74 & 3725.07
 & & 14.90 & 16.67  & 34886.45 & 8564.65
\\
\midrule
\multirow{5}*{pr1002}
 & 2 & 65541078 
 & & 5.99 & 52.28
 & & 0.35 & 0.99  & 215703.18 & 183435.59
 & & \textbf{0.00} & 0.63  & 227427.16 & 279021.00
\\
 & 4 & 36553749 
 & & 13.90 & 35.78
 & & 1.69 & 2.20  & 85095.75 & 53400.13
 & & \textbf{0.00} & 0.75  & 192716.60 & 81455.54
\\
 & 6 & 26676866 
 & & 9.48 & 36.38
 & & \textbf{0.00} & 0.28  & 33816.36 & 25943.29
 & & 1.17 & 2.10  & 318901.94 & 43332.34
\\
 & 8 & 20946133 
 & & 7.57 & 36.03
 & & \textbf{0.00} & 0.18  & 20700.88 & 14389.91
 & & 8.59 & 10.53  & 544729.91 & 30745.18
\\
 & 10 & 19540052 
 & & 6.21 & 37.82
 & & 0.96 & 1.14  & 17698.56 & 9307.68
 & & \textbf{0.00} & 3.34  & 524410.71 & 22968.16
\\
\midrule
\end{tabular}
\end{center}
\caption{Comparison of the algortihms for mTDP.}
\end{table*}

